Strong Khovanov-Floer Theories and Functoriality

We provide a unified framework for proving Reidemeister-invariance and functoriality for a wide range of link homology theories. These include Lee homology, Heegaard Floer homology of branched double covers, singular instanton homology, and \Szabo's geometric link homology theory. We follow Baldwin, Hedden, and Lobb (arXiv:1509.04691) in leveraging the relationships between these theories and Khovanov homology. We obtain stronger functoriality results by avoiding spectral sequences and instead showing that each theory factors through Bar-Natan's cobordism-theoretic link homology theory.

==> instantons.tex <==
		Our goal in this section is to suggest proofs that the gauge-theoretic Khovanov-Floer theories are strong.  Along the way, we define reduced strong Khovanov-Floer theories.

		In \cite{Kronheimer2011}, Kronheimer and Mrowka assign to a link diagram $\diagram$ with a basepoint $p$ a filtered complex $C(\diagram,p)$.

		\begin{Thm*}[Kronheimer, Mrowka \cite{Kronheimer2011}]
			Suppose that $\diagram$ is a diagram of the link $K$.  Let $p \in K$.  The homology of $C(\diagram,p)$ is the \emph{reduced instanton Floer homology} $I^\natural(K,p)$ of $K$.  The induced spectral sequence has $E_2 = \rKh(K,p)$, the \emph{reduced Khovanov homology of $K$} with basepoint $p$.
		\end{Thm*}

		We will not review the definitions of singular instanton knot homology or reduced Khovanov homology. (The latter is quite brief, see \cite{Khovanov2003}.)  

		We must adapt the definition of homotopy Khovanov-Floer theory to consider the basepoint.  A diagrammatic cobordism of pointed diagrams is defined exactly as for unpointed diagrams except that handles must be supported in the complement of a neighborhood of the basepoint.  The results of Section \ref{sec:diagrams} all apply, \emph{mutatis mutandis}, see \cite{BaldwinHeddenLobb2015}.

		\begin{Def}\label{def:rgkft}
			A \emph{pointed homotopy Khovanov-Floer theory (over $R$)} $\hkft$ is a rule which assigns to a pointed link diagram $(\diagram,p)$ and auxiliary data $A$ a filtered chain complex $\hkft(\diagram, A, p)$satisfying the following properties.
			\begin{enumerate}
				\item\label{rkft:coherence} Let $A_\al$ and $A_\be$ be two collections of auxiliary data.  Then the complexes $\hkft(\diagram,A_\al,p)$ and $\hkft(\diagram, A_\be,p)$ form a transitive system of filtered chain complexes up to homotopy.  Write $\hkft(\diagram,p)$ for the canonical representative.
				\item\label{rkft:crossingless} If $\diagram$ is a crossingless diagram of the unknot, then the homology of $\hkft(\diagram,p)$ is isomorphic to $XR$.
	            \item\label{rkft:kunneth} K\"{u}nneth formula for connected sum at the basepoint.
	        \end{enumerate}
	        A reduced homotopy Khovanov-Floer theory also assigns maps to diagrammatic cobordisms.  These maps must satisfy the following properties:
	        \begin{enumerate}[resume]
	            \item\label{rkft:handles} Suppose that $(\diagram',p)$ is obtained from $(\diagram,p)$ by a diagrammatic handle attachment.  Then for every collection of auxiliary data $A$ for $(\diagram,p)$ there is a collection $\phi(A)$ for $\diagram'$ so that
	            \[
	            	\handle[(A_{\al},\phi(A_{\al}),A_{\handle})] \co \hkft(\diagram,A_\al,p) \to \hkft(\diagram',\phi(A'_{\al'},p)).
	            \]
	            which depends on the auxiliary data for the diagrams along with possibly the extra data $A_{\handle}$.  These maps form a transitive system of maps over the first two pieces of auxiliary data and therefore induce a map
	            \[
	            	\handle \co \hkft(\diagram,p) \to \hkft(\diagram',p).
	            \]
	            There is a homotopy $\handle[(A_{\al},A_{\al'},A_{\handle}] \simeq \handle[(A_{\al},A_{\al'},A'_{\handle})]$ for any two sets of auxiliary data $A_{\handle}$ and $A'_{\handle}$.  
	            \item\label{kft:frobenius} For diagrammatic cobordisms of links without crossings, the handle maps agree on homology with those on $R$.  
				\item\label{kft:isotopy} If $\diagram'$ is obtained from $\diagram$ by a planar isotopy, then $\hkft(\diagram)$ is homotopy equivalent to $\hkft(\diagram')$.  If $\diagram$ is a crossingless diagram with one closed component, then this map is the identity.    
				\item\label{rkft:conditions} The handle attachment maps satisfy handleswap invariance and the movie move 15 relation.
			\end{enumerate}
		\end{Def}

		Let $\diagram$ be a pointed link diagram.  Then $I^\natural(\diagram \cup \circ) \cong I^{\natural} \otimes V$ with all the naturality one could ask for, see Section 8 of \cite{Kronheimer2011}.  It is shown in Section 2 of \cite{KronheimerMrowka} that this isomorphism can be achieved at chain homotopy level: there is a collection of analytic data so that the chain complex underlying $I^{\sharp}(\circ)$ is isomorphic to $V$ with vanishing differential.  So definitions of zero- and one-handle attachment maps are clear.

		\begin{Thm}\label{thm:instantons}
			There is a conic, pointed homotopy Khovanov-Floer theory $\hkft_I$ which assigns to pointed diagrams $(\diagram,p)$ the complex $C(\diagram,p)$.
		\end{Thm} 

		\begin{proof}(sketch)
		
			Condition 1 is discussed in Theorem 3.3 and the beginning of Section 5 of \cite{KronheimerMrowka}.  Condition 2 is Corollary 8.5 of \cite{Kronheimer2011}.  Condition 3 is implied by Corollary 5.9 of \cite{Kronheimer2011}.  

			Condition 4 is a combination of standard arguments and Theorem 3.3.  Condition 5 follows from Lemma 8.7 of \cite{Kronheimer2011} as well as the definition of the zero- and one-handle maps.  Condition 6 is Proposition 8.10 of \cite{Kronheimer2011}.  Condition \ref{rkft:handleKunneth} is Proposition 5.8 of \cite{Kronheimer2011} (so-called ``split naturality'').  The handleswap part of Condition \ref{rkft:conditions} is clear.

			Let $\Sigma$ be a 



		\end{proof}
		\begin{Rem}
			It is interesting to consider the four-dimensional geometry of the $S$ relation.  Let $\Sigma$ be a link cobordism which contains a closed sphere.  Then the double cover of $S^3 \times I$ branched along $\Sigma$ is a cobordism containing a homologically non-trivial sphere of self-intersection number zero.  This implies that the map assigned to this cobordism by any flavor of instanton Floer homology is zero \cite{Kronheimer1995}.  It is interesting to wonder whether the $T$ or even $4Tu$ relation can be given a similar treatment.
		\end{Rem}

		The proof for monopole Floer homology should be essentially the same.  Naturality is a (hard-fought) consequence of the construction of the theory in \cite{KronheimerMrowka}.  The construction of a conic theory is due to Bloom \cite{Bloom2011}.




